Stable Online Control of Linear Time-Varying Systems

Linear time-varying (LTV) systems are widely used for modeling real-world dynamical systems due to their generality and simplicity. Providing stability guarantees for LTV systems is one of the central problems in control theory. However, existing approaches that guarantee stability typically lead to significantly sub-optimal cumulative control cost in online settings where only current or short-term system information is available. In this work, we propose an efficient online control algorithm, COvariance Constrained Online Linear Quadratic (COCO-LQ) control, that guarantees input-to-state stability for a large class of LTV systems while also minimizing the control cost. The proposed method incorporates a state covariance constraint into the semi-definite programming (SDP) formulation of the LQ optimal controller. We empirically demonstrate the performance of COCO-LQ in both synthetic experiments and a power system frequency control example.

==> 5-Proof.tex <==
Our proof is mainly divided into two steps, 
\subsection{Proof of Lemma}
%We leverage the notion of strongly-stable and sequential strong stable policies introduced by~\cite{cohen2018online}, and extend it into the time-varying system setting. Intuitively, sequential strongly-stable policies are a sequence of policies, under which the norm of the state vectors remain controlled. 
% \begin{definition}{(strong stability)}
% A matrix $M$ is $(\kappa, \gamma)$-strongly stable (for $\kappa > 0$ and $0<\gamma\leq1$) if there exists matrices $H \succ 0$ and $L$ such that $M = HLH^{-1}$, with $\|L\| \leq 1-\gamma$ and $\|H\|\|H^{-1}\| \leq \kappa$.
% \end{definition}
% A policy $K_t$ for linear system $(A_t, B_t)$ is $(\kappa, \gamma)$-strongly stable (for $\kappa > 0$ and $0<\gamma\leq1$) if $\|K\| \leq \kappa$ and matrix $(A_t + B_t K_t)$ is $(\kappa, \gamma)$-strongly stable.
% \theoremstyle{definition}
% \begin{definition}{(sequential strong stability)}\label{def:str_seq_stab}
% A sequence of policies $K_1, K_2, ..., K_T$ such that $\pi(x_t) = K_t x_t$ for the linear time-varying dynamics $x_{t+1} = A_t x_t + B_t u_t$ is $(\kappa, \gamma, \rho)$-strongly stable (for $\kappa > 0$, $0<\gamma\leq 1$ and $0 \leq \rho < 1$) if there exist matrices $H_1, ..., H_T$ and $L_1, ..., L_T$ such that $A_t+B_tK_t = H_t L_t H_t^{-1}$ for all $t$, with the following properties:
% \begin{itemize}
%     \item $\|L_t\| \leq 1-\gamma$ and $\|K_t\| \leq \kappa$;
%     \item $\|H_t\| \leq \beta$ and $\|H_t^{-1}\| \leq 1/\alpha$ with $\kappa = \beta/\alpha$; \guannan{ABUSE OF NOTATION HERE. FIX LATER. }
%     \item $\|H_{t+1}^{-1} H_t\| \leq \frac{\rho}{1-\gamma}$.
% \end{itemize}
% \end{definition}

For a sequentially strongly stable sequence of policies, we can show that the magnitude of state remain controlled as the following lemma.
\begin{lemma}
Let $x_1, x_2, ...$ be a sequence of states starting from initial state $x_1$, and generated by the dynamics in Eq~\eqref{eq:lti_dyn} following a $(\kappa, \gamma, \rho)$-strongly stable sequence of policies $K_1, K_2, ...$. Then, for all $t \geq t_0\geq 1$ we have,
$$\|x_t\| \leq \kappa \rho^{t-t_0} \|x_{t_0}\| + \frac{\kappa \rho}{1-\rho} \max_{t_0 \leq s <t}\|w_s\|\,,$$
\end{lemma}
\begin{proof}
We prove the Lemma for the case where $t_0 = 1$. The proof for general $t_0$ is almost the same with slightly heavier notation. Since $u_t = K_t x_t$, we have $x_{t+1} = A_t x_t + B_t u_t + w_t= (A_t+B_t K_t)x_t + w_t$. Thus,
$$x_t = M_1 x_1 + \sum_{s=1}^{t-1} M_{s+1} w_s\,,$$
where 
$$M_t = I; M_s=M_{s+1}(A_s+B_s K_s) = (A_{t-1}+B_{t-1}K_{t-1}) \cdots (A_{s}+B_s K_s). %\,, \forall 1 \leq s \leq t-1.
$$

By the strong sequential stability, there exist matrices $H_1, H_2,...$ and $L_1, L_2, ...$ such that $A_j + B_j K_j = H_j L_j H_j^{-1}$, and $H_j, L_j$ satisfy the properties specified in Definition~\ref{def:str_seq_stab}. Thus we have for all $1 \leq s < t$,
\begin{align*}
    \| M_s \| &= \| H_{t-1} L_{t-1} H_{t-1}^{-1} H_{t-2} L_{t-1} H_{t-2}^{-1} \cdots H_s L_s H_s^{-1} \| \\
    & \leq \|H_{t-1}\| \left(\prod_{j=s}^{t-1} \|L_{j}\|\right) \left(\prod_{j=s}^{t-2} \|H_{j+1}^{-1} H_j\| \right) \|H_s^{-1}\|\,,\\
    & \leq \beta (1-\gamma)^{t-s} (\frac{\rho}{1-\gamma})^{t-s} (1/\alpha)\,, \\
    &\leq \kappa \rho^{t-s} 
\end{align*}
As $\kappa \geq 1$, the same holds for $M_t$. Thus, we have, 
\begin{align*}
    \| x_t \| &\leq \| M_1 \|  \| x_1\| + \sum_{s=1}^{t-1} \| M_{s+1}\| \|w_s\| \\
    & \leq \kappa \rho^{t-1} \|x_1\| + \kappa \sum_{s=1}^{t-1} \rho^{t-s-1} \|w_s\| \\
    & \leq \kappa \rho^{t-1} \|x_1\| + \kappa \max_{1 \leq s <t}\|w_s\| \sum_{t=1}^{\infty} \rho^{t}\\
    & = \kappa \rho^{t-1} \|x_1\| + \frac{\kappa \rho}{1-\rho} \max_{1 \leq s <t}\|w_s\|.
\end{align*}
\end{proof}


\begin{theorem}
Let $\Sigma_1, \Sigma_2, ...$ be the optimal solutions to the SDP in Algorithm~\ref{alg1}, and $K_1, K_2, ...$ are the associated sequence of control policies. Suppose that $0 \leq \alpha \leq \frac{1}{2}$, then the sequence $K_1, K_2, ...$ is $(\kappa, \gamma, \rho)$-sequentially strongly stable.
\end{theorem}

The proof is given by combining the following four lemmas. Lemma~\ref{lemma0} shows that the optimization problem in~\eqref{sdp_lqr_wconst} is always feasible for $0\leq \alpha <1$ and Lemma~\ref{lemma1} shows that the optimal control policy can be extracted from the SDP solution $\Sigma$, as $u_t = K_t x_t$ and $K_t = \Sigma_{xu}^{\top} \Sigma_{xx}^{-1}$.
\begin{lemma}\label{lemma0}
When $B$ is invertible, the SDP~\eqref{sdp_lqr_wconst} is always feasible for any $\alpha \in [0, 1)$.
\end{lemma}
\begin{proof}
We prove the lemma by explicitly constructing a feasible solution for ~\eqref{sdp_lqr_wconst}. 

Let $\Sigma_0 = \begin{bmatrix}W & -WA_t^{\top} (B_t^{-1})^{\top}\\
-B_t^{-1}A_tW & B_t^{-1}A_tWA_t^{\top}(B_t^{-1})^{\top}\end{bmatrix}$. It suffices to show that for $\alpha=0$, $\Sigma_0$ satisfies~\eqref{eq:const_stationary},~\eqref{eq:positivedef} and~\eqref{eq:const_stability}. 

Firstly, $\begin{bmatrix} A_t & B_t\end{bmatrix} \Sigma_0 \begin{bmatrix} A_t & B_t\end{bmatrix}^{\top} = \begin{bmatrix} A_t & B_t\end{bmatrix}\begin{bmatrix}W & -WA_t^{\top} (B_t^{-1})^{\top}\\
-B_t^{-1}A_tW & B_t^{-1}A_tWA_t^{\top}(B_t^{-1})^{\top}\end{bmatrix}\begin{bmatrix} A_t & B_t\end{bmatrix}^{\top} = 0$, thus constraint~\eqref{eq:const_stability} holds.

Plugging in $\begin{bmatrix} A_t & B_t\end{bmatrix} \Sigma_0 \begin{bmatrix} A_t & B_t\end{bmatrix}^{\top} = 0$ to~\eqref{eq:const_stationary}, $\Sigma_{xx} = W$ holds by the construction of $\Sigma_0$.

Finally, using the Schur complement condition for positive semi-definiteness, 
$$W \succ 0$$
$$B_t^{-1}A_tWA_t^{\top}(B_t^{-1})^{\top} - B_t^{-1}A_tWW^{-1}WA_t^{\top} (B_t^{-1})^{\top} = 0$$
thus $\Sigma_0 \succeq 0$ and constraint~\eqref{eq:positivedef} holds.
\end{proof}
\begin{lemma}\label{lemma1}
Suppose $Q,R,W$ are strictly positive definite and $\alpha\in[0,1)$. If \eqref{sdp_lqr_wconst} has a minimizer $\Sigma^*$, then there exists $K\in\mathbb{R}^{p\times n}$ s.t. $\Sigma^*$ can be written as  
\begin{align*}
 \Sigma^*= \begin{bmatrix}\Sigma_{xx}^{*} & \Sigma_{xu}^{*}\\
 {\Sigma_{ux}^{\top}} & \Sigma_{uu}^{*}\end{bmatrix} = \begin{bmatrix}\Sigma_{xx}^{*} & \Sigma_{xx}^{*} K^{\top}\\
K \Sigma_{xx}^{*} & K \Sigma_{xx}^{*} K^{\top} \end{bmatrix}
\end{align*}
\end{lemma}
\begin{proof}
Clearly, $\Sigma_{xx}^* \succeq W \succ 0$, and therefore we can simply define $K = \Sigma_{ux}^*(\Sigma_{xx}^*)^{-1}$, and the only thing we need to show is $\Sigma_{uu}^* = K \Sigma_{xx}^{*} K^{\top}$. Suppose this is not true, then since $\Sigma^*\succeq 0$, there must exist $D\neq 0, D\succeq 0$ s.t. 
\begin{align}
    \Sigma_{uu}^* = K \Sigma_{xx}^{*} K^{\top} + D.
\end{align}
Then, by \eqref{eq:const_stationary}, we also have,
\begin{align}
    \Sigma_{xx}^* = (A_t + B_t K)\Sigma_{xx}^* (A_t+ B_tK)^{\top} + B_t D B_t^{\top}  + W. \label{eq:realizability:sigmaxx}
\end{align}  
Viewing the above as a Lyapunov equation in terms of $\Sigma_{xx}^*$, and since $B_t D B_t^{\top} + W\succ 0$ and $\Sigma_{xx}^*\succ 0$, we get $A_t + B_t K$ is a stable matrix. 

Next, since $A_t + B_t K$ is stable, we can construct $\tilde{\Sigma}_{xx}$ to be the unique solution to the following Lyapunov equation,
\begin{align}
    \tilde\Sigma_{xx} = (A_t + B_t K)\tilde\Sigma_{xx} (A_t+ B_tK)^{\top}  + W. \label{eq:realizability:tildesigmaxx}. 
\end{align}
We further define,
\begin{align*}
 \tilde{\Sigma}=\begin{bmatrix}\tilde\Sigma_{xx} & \tilde\Sigma_{xx} K^{\top}\\
K \tilde\Sigma_{xx} & K \tilde\Sigma_{xx} K^{\top} \end{bmatrix},
\end{align*}
and we claim that $\tilde\Sigma$ is a feasible solution to \eqref{sdp_lqr_wconst}. Clearly $\tilde{\Sigma}$ is positive semi-definte, and further, it satisfies \eqref{eq:const_stationary}. We now check that \eqref{eq:const_stability} is met. For this purpose, we have,
\begin{align*}
    &\begin{bmatrix} A_t & B_t\end{bmatrix} \tilde\Sigma \begin{bmatrix} A_t & B_t\end{bmatrix}^\top - \alpha \tilde{\Sigma}_{xx} \\
    &=( A_t + B_t K)\tilde{\Sigma}_{xx} (A_t + B_tK)^\top - \alpha \tilde{\Sigma}_{xx}\\
    &= ( A_t + B_t K){\Sigma}_{xx}^* (A_t + B_tK)^\top - \alpha {\Sigma}_{xx}^* + ( A_t + B_t K) ( \tilde{\Sigma}_{xx} -  {\Sigma}_{xx}^* ) (A_t + B_tK)^\top - \alpha( \tilde{\Sigma}_{xx} -  {\Sigma}_{xx}^*)\\
    &\preceq - B_t D B_t^\top + ( A_t + B_t K) ( \tilde{\Sigma}_{xx} -  {\Sigma}_{xx}^* ) (A_t + B_tK)^\top - \alpha( \tilde{\Sigma}_{xx} -  {\Sigma}_{xx}^*), \end{align*}
    where the last step is due to $\Sigma^*$ must satisfy \eqref{eq:const_stability}. 
    Subtracting \eqref{eq:realizability:sigmaxx} from \eqref{eq:realizability:tildesigmaxx}, we have,
  \[  \tilde{\Sigma}_{xx} - \Sigma_{xx}^* =  ( A_t + B_t K) ( \tilde{\Sigma}_{xx} -  {\Sigma}_{xx}^* ) (A_t + B_tK)^\top  - B_t D B_t^\top.   \]
  Since $A_t + B_tK$ is stable, and $B_t D B_t^\top \neq 0$ (since $D\neq 0$, $B_t$ invertable), we have $\tilde{\Sigma}_{xx} - \Sigma_{xx}^* \preceq 0$, and $\tilde{\Sigma}_{xx} - \Sigma_{xx}^* \neq 0$. As such, we have
  \begin{align*}
          \begin{bmatrix} A_t & B_t\end{bmatrix} \tilde\Sigma \begin{bmatrix} A_t & B_t\end{bmatrix}^\top - \alpha \tilde{\Sigma}_{xx} 
    \preceq (1-\alpha) (\tilde{\Sigma}_{xx} - \Sigma_{xx}^*) \preceq 0.
  \end{align*}
  This shows $\tilde{\Sigma}_{xx} $ is a feasible solution to \eqref{sdp_lqr_wconst}. Further, one can easily check  $\tilde{\Sigma}_{xx} $ achieves a strictly lower cost due to $Q,R$ are strictly positive definite. So we get a contradiction, and the proof is concluded. 
\end{proof}

Next, we show that each policy $K_t$ is strongly stable.
\begin{lemma}\label{lemma2}
$K_t$ is $(\kappa, \gamma)$-strongly stable for $A_t + B_t = H_t L_t H_t^{-1}$, with $\|L_t\| \leq \sqrt{\alpha}$ and $\|H_t\| \|H_t^{-1}\| \leq \frac{1}{\sqrt{1-\alpha}}$.
\end{lemma}
\begin{proof}
First, we re-write the left side of constraint~\eqref{eq:const_stability} as follows,
\begin{align*}
    \begin{bmatrix} A_t & B_t\end{bmatrix} \Sigma \begin{bmatrix} A_t & B_t\end{bmatrix}^{\top} &= \begin{bmatrix} A_t & B_t\end{bmatrix} \begin{bmatrix}\Sigma_{xx} & \Sigma_{xx}K_t^{\top}\\ K_t\Sigma_{xx} & K_t\Sigma_{xx}K_t^{\top}\end{bmatrix} \begin{bmatrix} A_t^{\top} \\ B_t^{\top}\end{bmatrix} \\
    &= A_t \Sigma_{xx} A_t^{\top} + A_t K_t\Sigma_{xx} B_t^{\top}+B_t\Sigma_{xx} K_t^{\top} A_t^{\top} + B_t K_t \Sigma_{xx} K_t^{\top} B_t^{\top} \\
    &= (A_t+B_tK_t) \Sigma_{xx} (A_t+B_t K_t)^{\top}
\end{align*}

Therefore, ~\eqref{eq:const_stability} can be equivalently expressed as,
\begin{equation}
    (A_t+B_tK_t) \Sigma_{xx} (A_t+B_t K_t)^{\top} \leq \alpha \Sigma_{xx}\,,
\end{equation}

Left multiplying $\Sigma_{xx}^{-1/2}$ and right multiplying $\Sigma_{xx}^{-1/2}$,
\begin{equation}\label{eq:lt_bound}
\Sigma_{xx}^{-1/2} (A_t+B_tK_t) \Sigma_{xx}^{1/2} \Sigma_{xx}^{1/2} (A_t+B_t K_t)^{\top} \Sigma_{xx}^{-1/2} \leq \alpha I\,,
\end{equation}

Let $H_t = \Sigma_{xx}^{1/2}$, $L_t = \Sigma_{xx}^{-1/2} (A_t+B_tK_t) \Sigma_{xx}^{1/2}$, which gives us the following decomposition,
$$(A_t+B_tK_t) = H_t L_t H_t^{-1}\,,$$

Eq~\eqref{eq:lt_bound} provides an upper bound on $\|L_t\|$. $L_t L_t^{\top} \leq \alpha I$, thus $\|L_t\| \leq \sqrt{\alpha} \in [0, 1)$. 

To derive the bound on $\|H_t\| \|H_t^{-1}\|$, we plug in $\begin{bmatrix} A_t & B_t\end{bmatrix} \Sigma \begin{bmatrix} A_t & B_t\end{bmatrix}^{\top} = \Sigma_{xx}-W$ from Eq.~\eqref{eq:const_stationary} into~s\eqref{eq:const_stability}, which implies,
$$\Sigma_{xx}- W \leq \alpha \Sigma_{xx}, \alpha \in [0, 1)\,,$$
Equivalently,
$$W \leq \Sigma_{xx} \leq \frac{W}{1-\alpha}.$$

Therefore, $\|H_t\| = \|\Sigma_{xx}^{1/2}\| \leq \frac{\|W^{1/2}\|}{\sqrt{1-\alpha}}$, $\|H_t^{-1}\| = \|\Sigma_{xx}^{-1/2}\| \leq {\|W^{-1/2}\|}$, $\|H_t\| \|H_t^{-1}\| \leq \frac{\| W^{1/2}\| \| W^{-1/2}\|}{\sqrt{1-\alpha}}$. \guannan{to-do: change to $W = I$... }

Thus, $(A_t+B_t K_t)$ is $(\kappa, \gamma)$ strongly stable, for $\gamma = 1-\sqrt{\alpha}$ and $\kappa = \frac{1}{\sqrt{1-\alpha}}$.
\end{proof}

Furthermore, having established strong stability, the next lemma shows that the sequence of policies are sequentially strongly stable for $0 \leq \alpha < \frac{1}{2}$.
\begin{lemma}\label{lemma3}
For all $0 \leq \alpha \leq \frac{1}{2}$, there exists $\rho \in [0, 1)$ such that $\|H_{t+1}^{-1} H_t\| \leq \frac{\rho}{1-\gamma}$.
\end{lemma}
\begin{proof}
We show that the conditions for sequential strong-stability hold for $\alpha < \frac{1}{2}$. Notice that Lemma~\ref{lemma2} show that for all $t$, $K_t$ is $(\kappa, \gamma)$-strongly stable, it also gives us a uniform upper and lower bound on $H_t = \Sigma_{xx}^{1/2}$ as $\|W^{1/2}\| \leq \|\Sigma_{xx}^{1/2}\| \leq \frac{\|W^{1/2}\|}{\sqrt{1-\alpha}}$, and $$\|H_{t+1}^{-1} H_t\| \leq \frac{1}{\sqrt{1-\alpha}}$$.

Together with sequential strong stability definition, that $\|H_{t+1}^{-1} H_t\| \leq \frac{\rho}{1-\gamma}$ for $\rho \in [0, 1)$. A sufficient condition for sequential strong stability is to ensure that,
$$\frac{1}{\sqrt{1-\alpha}} \leq \frac{1}{1-\gamma}\,,$$
where $\gamma = 1-\sqrt{\alpha}$. Thus $0 \leq \alpha \leq \frac{1}{2}$ provides sequential strong-stability.
\end{proof}

